Methods for Ordinal Peer Grading

MOOCs have the potential to revolutionize higher education with their wide outreach and accessibility, but they require instructors to come up with scalable alternates to traditional student evaluation. Peer grading -- having students assess each other -- is a promising approach to tackling the problem of evaluation at scale, since the number of "graders" naturally scales with the number of students. However, students are not trained in grading, which means that one cannot expect the same level of grading skills as in traditional settings. Drawing on broad evidence that ordinal feedback is easier to provide and more reliable than cardinal feedback, it is therefore desirable to allow peer graders to make ordinal statements (e.g. "project X is better than project Y") and not require them to make cardinal statements (e.g. "project X is a B-"). Thus, in this paper we study the problem of automatically inferring student grades from ordinal peer feedback, as opposed to existing methods that require cardinal peer feedback. We formulate the ordinal peer grading problem as a type of rank aggregation problem, and explore several probabilistic models under which to estimate student grades and grader reliability. We study the applicability of these methods using peer grading data collected from a real class -- with instructor and TA grades as a baseline -- and demonstrate the efficacy of ordinal feedback techniques in comparison to existing cardinal peer grading methods. Finally, we compare these peer-grading techniques to traditional evaluation techniques.

==> discussion.tex <==
\section{Discussion}

Note that the model we consider is general enough to accommodate common extensions observed in practice:
\begin{itemize}
 \item {\bf External Graders:} Our model does not restrict the graders to necessarily be students. Thus we can incorporate expert graders \ie course staff/instructors (and model their reliabilities with stronger priors), or other external reviewers in our model as well.
 \item {\bf Self-Grading:} Another popular evaluation practice is self-assessment. When performed in conjunction with peer evaluation this has been found to instructional and has led to greater objectivity in the self-assessments \cite{sung_selfpeer_2005}. Self-assessment is trivially incorporated in our framework; furthermore, by tying it to the grader reliability, this also incentivizes objectivity and honesty in the self-evaluation.
 \item {\bf Peer-Reviewing:} Our model can also be used for conference reviewing, which follows a similar system as that used in peer grading.
\end{itemize}
- Can be extended to active learning.

==> experiment-conventional.tex <==
\section{Comparison to conventional grading practices}


- Grader rating change before and after seeing student reviews (Meta-Reviews) for PPo and FR.

\begin{table}[t]
\footnotesize
\addtolength{\tabcolsep}{-0.75mm}
\centering
 \begin{tabular}{|c||c|c|c|}
 \hline
   & \multicolumn{3}{c|}{ {\bf Grader A} } \\ \hline
  {\bf Grader B}  & $d_1 \succ d_2$ & $d_1 \approx d_2$ & $d_1 \prec d_2$ \\ \hline
   $d_1 \succ d_2$ & 19 & 9 & 14\\ 
   $d_1 \approx d_2$ & - & 1 & 3\\ 
 \hline
\end{tabular}
\caption{\label{tab:ppo-self-agreement} Agreement for PPO which is equivalent to having $\expct[\delta_{KT}(\cdot,\cdot)]=0.436$ }
\end{table}
% 19 + 4.5 + 14 + 1.5 = 39
% 2.25 + 14 + 0.75 = 17
% 17/39 = 0.436




\begin{table}[t]
\footnotesize
\addtolength{\tabcolsep}{-0.75mm}
\centering
 \begin{tabular}{|c||c|c|c|}
 \hline
   & \multicolumn{3}{c|}{ {\bf Grader A} } \\ \hline
  {\bf Grader B}  & $d_1 \succ d_2$ & $d_1 \approx d_2$ & $d_1 \prec d_2$ \\ \hline
   $d_1 \succ d_2$ & 12 & 7 & 2\\ 
   $d_1 \approx d_2$ & - & 4 & 2\\ 
 \hline
\end{tabular}
\caption{\label{tab:fr-self-agreement} Agreement for FR  which is equivalent to having $\expct[\delta_{KT}(\cdot,\cdot)]=0.230$}
\end{table}
% 12 + 3.5 + 2 + 1 = 18.5
% 1.75 + 2 + 0.5 = 4.25
% 8.5/37 = 0.230


Conventional grading practices involves the course staff (TAs/Instructors) manually going through each assignment laboriously.
With larger classes and larger student-to-staff ratios, this can become increasingly hard and time-consuming (consequently leading to more errors as well).
To avoid such {\em fatigue}, we had each member of the course staff review $\approx 11$ posters and $\approx 9$ final reports on average (we did not this for the proposal stage).
This resulted in having 46 overlapping pairs for the poster dataset and 27 for the final reports.

To gage how our results compare to these conventional practices, we calculated the agreement between the reviewers for such overlapping pairs.
The resuls are shown in Tables~\ref{tab:ppo-self-agreement} and \ref{tab:fr-self-agreement}.
While for the posters there is a larger disagreement (due to the differing quality of the different presenters of the posters) with $\expct[\delta_{KT}(\cdot,\cdot)]=0.436$, even for the final reports we find an expected Kendall tau (with ties) of 0.23, which is comparable with the results of the different OPG methods we studied.
In summary, we find that our OPG methods are able to achieve ranking agreement with staff rankings comparable to that of the inter-staff ranking agreement.


\begin{table}[t]
\footnotesize
\addtolength{\tabcolsep}{-0.75mm}
\centering
 \begin{tabular}{|c||c|c|c|}
 \hline
   & \multicolumn{3}{c|}{ {\bf TAs} (T) } \\ \hline
  {\bf Instructor} (I)  & $d_1 \succ d_2$ & $d_1 \approx d_2$ & $d_1 \prec d_2$ \\ \hline
   $d_1 \succ d_2$ & 84 & 19 & 7\\ 
   $d_1 \approx d_2$ & 15 & 16 & 9\\ 
 \hline
\end{tabular}
\caption{\label{tab:ppo-cross-agreement} Cross-Agreement for PO: $\expct[\delta_{KT}(\ordering_I,\ordering_T)]=0.150$ and (if ties broken randomly) $\expct[\delta_{K}(\ordering_I,\ordering_T)]=0.243$.}
\end{table}

%Numer = 9.5 + 7
%Denom  = 84 + 19 + 7
%Numer = 9.5 + 7 + 7.5 + 8 + 4.5
%Denom  = 84 + 19 + 7 + 15 + 16 + 9


\begin{table}[t]
\footnotesize
\addtolength{\tabcolsep}{-0.75mm}
\centering
 \begin{tabular}{|c||c|c|c|}
 \hline
   & \multicolumn{3}{c|}{ {\bf TAs} (T) } \\ \hline
  {\bf Instructor} (I)  & $d_1 \succ d_2$ & $d_1 \approx d_2$ & $d_1 \prec d_2$ \\ \hline
   $d_1 \succ d_2$ & 121 & 33 & 13\\ 
   $d_1 \approx d_2$ & 25 & 28 & 28\\ 
 \hline
\end{tabular}
\caption{\label{tab:fr-cross-agreement} Cross-Agreement for FR $\expct[\delta_{KT}(\ordering_I,\ordering_T)]=0.177$ and (if ties broken randomly) $\expct[\delta_{K}(\ordering_I,\ordering_T)]=0.282$.}
\end{table}

%Numer = 16.5 + 13
%Denom  = 121 + 33 + 13
%Numer = 16.5 + 13 + 12.5 + 14 + 14
%Denom  = 121 + 33 + 13 + 25 + 28 + 28


While is impossible to obtain {\em true gold standard} rankings for the assignemnts, we tried to obtain a {\em silver} standard via the meta-review stage.
For the proposals this involved having a dedicated TA go over all the different reviews for the assingments and determine the grades.
For the final reports, the two authors as the project staff leads, split the assignments in half and reviewed the different assignments while also considering the reviews from the other staff (but not the student reviews).
While both of these stages utilized the staff reviews, we still would like to roughly estimate how accurate the staff rankings are compared to these silver standard rankings.

The results of this comparison are shown in Tables~\ref{tab:ppo-cross-agreement} and \ref{tab:fr-cross-agreement}.
As we see even the staff rankings differ considerably with $\expct[\delta_{KT}(\cdot,\cdot)]$ between 15-20\%.

==> experiment-scores.tex <==

\begin{table}[t]
\scriptsize
\addtolength{\tabcolsep}{-1.25mm}
\centering
%  \begin{tabular}{|c|c|c|}
%  \hline
%    Method & MAE & RMSE \\ \hline
% \multicolumn{3}{|c}{PR} \\ \hline
% SCAVG & 0.51  & 0.65 \\
% NCS & 0.50  & 0.64 \\
% MAL & 0.49  & 0.65 \\
% MAL$_{BC}$ & 0.49  & 0.64 \\
% LP & 0.49  & 0.64 \\
% NP & 0.51  & 0.66 \\
% CLR & 0.50  & 0.64 \\
% SWDS & 0.56  & 0.73 \\
% SWDR & 0.53  & 0.72 \\
%  \hline
% \end{tabular}
 \begin{tabular}{|c|cc|cc|}
 \hline
   Method & \multicolumn{2}{c|}{Poster} & \multicolumn{2}{c|}{Report}   \\ \cline{2-5}
   & MAE & RMSE & MAE & RMSE  \\ \hline
   SCAVG & 0.60  & 0.76  & 0.74  & 1.00 \\
NCS & 0.64  & 0.78  & 0.84  & 1.15 \\
% MAL & 0.70  & 0.87  & 0.87  & 1.15 \\
% MAL$_{BC}$ & 0.71  & 0.84  & 0.85  & 1.15 \\
MALS & 0.63  & 0.81  & 0.89  & 1.18 \\  
BT & 0.64  & 0.78  & 0.90  & 1.24 \\
THUR & 0.64  & 0.78  & 0.92  & 1.29 \\
PL & 0.68  & 0.83  & 0.89  & 1.23 \\
% SWDS & 0.63  & 0.85  & 0.89  & 1.19 \\
% SWDR & 0.63  & 0.81  & 0.89  & 1.18 \\  
\hline
TAs & 0.66  & 0.98  & 0.73  & 0.96 \\  \hline
% SCAVG & 0.60  & 0.76 \\
% NCS & 0.64  & 0.78 \\
% MAL & 0.70  & 0.87 \\
% MAL$_{BC}$ & 0.71  & 0.84 \\
% LP & 0.64  & 0.78 \\
% NP & 0.64  & 0.78 \\
% CLR & 0.68  & 0.83 \\
% SWDS & 0.63  & 0.85 \\
% SWDR & 0.63  & 0.81 \\
% \hline
% \end{tabular}
%  \begin{tabular}{|c|c|c|}
%  \hline
%    Method & MAE & RMSE \\ \hline
% \multicolumn{3}{|c|}{FR} \\ \hline
% SCAVG & 0.74  & 1.00 \\
% NCS & 0.84  & 1.15 \\
% MAL & 0.87  & 1.15 \\
% MAL$_{BC}$ & 0.85  & 1.15 \\
% LP & 0.90  & 1.24 \\
% NP & 0.92  & 1.29 \\
% CLR & 0.89  & 1.23 \\
% SWDS & 0.89  & 1.19 \\
% SWDR & 0.89  & 1.18 \\
% \hline
\end{tabular}
\caption{\label{tab:exp_score_recovery} Cardinal error measures indicating how well the peer grading methods (\& TAs) predict the Instructor/Meta grades.}
\end{table}


\subsection{Can Ordinal Peer Grading Methods Estimate Cardinal Grades?}
\label{sec:exp_scores}
While the previous sections showed that the ordinal peer grading methods are able to predict the assignment ordering quite well, in this section we explore how well they do at predicting cardinal grades.
We first rescale the grades output by the different methods ($\cardinalest{d}$) to have identical mean and deviation as the instructor/meta grades to make all the scores comparable.
We measure the Mean Absolute Error (MAE) and Root Mean Squared Error (RMSE) for these rescaled scores, using the instructor/meta grades as labels.

The results are shown in Table~\ref{tab:exp_score_recovery}.
The results indicate that, despite not receiving any cardinal feedback, the OPG techniques are able to predict meta/instructor grades nearly as well as the cardinal peer grading methods.
Furthermore, when performing the same rescaling and metric computation for the TA grades, we find that these peer-grading methods do comparably to the TA performance as well.
This only further exemplifies the suitability of these techniques as a replacement to conventional grading techniques.



\longversion{
RMSE values for the synth data
}
